CLVSA: A Convolutional LSTM Based Variational Sequence-to-Sequence Model with Attention for Predicting Trends of Financial Markets

Financial markets are a complex dynamical system. The complexity comes from the interaction between a market and its participants, in other words, the integrated outcome of activities of the entire participants determines the markets trend, while the markets trend affects activities of participants. These interwoven interactions make financial markets keep evolving. Inspired by stochastic recurrent models that successfully capture variability observed in natural sequential data such as speech and video, we propose CLVSA, a hybrid model that consists of stochastic recurrent networks, the sequence-to-sequence architecture, the self- and inter-attention mechanism, and convolutional LSTM units to capture variationally underlying features in raw financial trading data. Our model outperforms basic models, such as convolutional neural network, vanilla LSTM network, and sequence-to-sequence model with attention, based on backtesting results of six futures from January 2010 to December 2017. Our experimental results show that, by introducing an approximate posterior, CLVSA takes advantage of an extra regularizer based on the Kullback-Leibler divergence to prevent itself from overfitting traps.

==> model_bk.tex <==
\section{Model design}\label{model}
The architecture of our proposed model, CLVSA, is illustrated in Figure \ref{fig:CLVSA}. The 2-layer encoder and decoder of the sequence-to-sequence framework take 2-D data frames of two consecutive days, respectively. Convolutional LSTM units process 
2-D data frames by two steps: i) Convolutional kernels capture local features, ii) Based on the local features, LSTM networks capture temporal features with gated recurrent networks. In each layer of the encoder and decoder, we have a self-attention module to highlight parts of the sequence of daily data frames. We also have an inter-attention module to highlight parts of the first one of two consecutive days as the context of the second day. The backward decoder takes the reversed 2-D data frames of the second day for generating the KLD based regularizer.

%It mainly consists of a sequence-to-sequence framework that includes an encoder and decoder, an extra backward decoder, an inter-attention module, two projection layers, and two feed-forward networks for the reparameterization trick \cite{kingma2013auto}. The encoder, decoder and backward decoder have two layers, each of layers consists of a convolutional LSTM unit and a self-attention module. The inter-attention module provide the weighted sum of final states of the encoder to the two layers of the decoder. 

%We assemble Convolutional LSTM units, Sequence-to-sequence framework with attention mechanisms, and a backward decoder for the approximate posterior into our proposed model, CLVSA, whose architecture is illustrated in Figure \ref{fig:CLVSA}. We describe each component in the following subsections:

\begin{figure}
\centering
\includegraphics[width=1\linewidth]{img/convLSTM.pdf}
\caption{\textbf{The architecture of the Convolutional LSTM unit}}
\label{fig:convLSTM}
\end{figure}

\subsection{Convolutional LSTM units}
All hidden layers In vanilla LSTM network \cite{hochreiter1997long} are fully connected layers, it works well for tasks such as speech recognition and natural language processing because we can perfectly map speeches and texts into trainable vector space \cite{mikolov2013distributed}, however, it struggles with the other tasks of which purely numeric data can not tokenized. Convolutional LSTM units addresses this issue by replacing fully connected layers with convolutional kernels. Formally,
\begin{equation}
\begin{gathered}\label{eq:convlstm}
i_{t} = \sigma(W_{i}*[X_{t},H_{t-1}] + b_{i}) \\
f_{t} = \sigma(W_{f}*[X_{t},H_{t-1}] + b_{f}) \\
o_{t} = \sigma(W_{o}*[X_{t},H_{t-1}] + b_{o}) \\
C_{t} = f_{t} \circ C_{t-1} + i_{t} \circ \tanh(W_{c}*[X_{t},H_{t-1}] + b_{c}) \\
H_{t} = o_{t} \circ \tanh(C_{t})
\end{gathered}
\end{equation}
where $X_{t}$, $H_{t}$, $C_{t}$ denote the input data, hidden state, and cell state at time step $t$, respectively; $i_{t}$, $f_{t}$, $o_{t}$ denote the output of the input, forget, and output gate at time step $t$; $W_{i}$, $W_{f}$, $W_{o}$ denote the convolutional kernels of the input, forget, and output gate; $b_{i}$, $b_{f}$, $b_{o}$ denote the bias of the input, forget, and output gate. The symbol $*$ denotes the convolution operator and $\circ$ denotes the point-wise product operation. Since parameters sharing is the key factor for generalization of deep learning models, with the convolutional operations between the kernels and data, parameters of the kernels are shared among input data so that convolution is more powerful to extract generalized features from data.

However, we can not directly use the original design of convolutional LSTM units due to the property of financial trading data. Although trading data can be organized into 2-D frames, we can not apply 2-D convolutions because the rows of the 2-D frames contains different types of features including Open, High, Low, Close price, and Volume. Instead we use a modified version of 1-D convolution: kernels only move horizontally across columns, the time line of 2-D data frames, while they are also shared among different types of data to guarantee parameters sharing. The unfolding view of convolutional LSTM network is illustrated in Figure \ref{fig:convLSTM}. Note that we follow the design in \cite{xingjian2015convolutional} that we do not compress the size of input frames during convolutions, that means if input frames $X_{t}$ are 6x5 and output channels are 32, then the final hidden state output $H_{t}$ should be 6x5x32 and they are flattened to a vector as the input of the subsequent classifier layer.

\begin{figure*}
\centering
\includegraphics[width=1\linewidth]{img/CLVSA.pdf}
\caption{\textbf{The architecture of CLVSA.} Both the encoder and decoder of the sequence-to-sequence framework have two layers, each of the layers applies a convolutional LSTM unit and a self-attention module. The inter-attention module communicates the final layer of the encoder, to the both layers of the forward decoder. Since there exist interactions between convolutional LSTM units and attention modules, we use double sided arrows to connect them.}
\label{fig:CLVSA}
\end{figure*}

\subsection{Sequence-to-sequence framework With attention mechanisms}
There are two main motivations to use sequence-to-sequence framework with attention mechanisms (illustrated in Figure \ref{fig:CLVSA}) as the foundation of our model. First, trading volume has a significant rhythmicity. Take futures markets for instance, in every regular trading day, the quantity of trades keeps low in the midnight, starts to slowly increase in the early morning, reaches a plateau from 9am to 2pm around, and then quickly falls to the low ebb (as showed in Figure \ref{fig:yahoo}), the trading volume (the bottom bar charts) of light sweet crude oil futures (CL) on Jan 23, 2019 and Jan 24, 2019. Second, although longer sequence may provide more context information, training long sequences may make cross entropies too large for the model to converge due to the noisy and dynamic characteristics of financial markets. We thus split trading data into segments by individual days to fit the above regularity, then feed trading data of two consecutive days to the encoder and decoder, respectively.

We use the inter-attention mechanism \cite{bahdanau2014neural} to strengthen the connection between the encoder and decoder. The basic idea is that, at time step $t_{d}$ of the decoder, we concatenate its hidden state $hd_{t_{d}}$ with the weighted average of hidden states of the encoder. The weight of each time step $t_{e}$ of the encoder is determined by the similarity between $he_{t_{e}}$ and $hd_{t_{d}}$. Formally,
\begin{equation}
\begin{gathered}\label{eq:inter-attention}
ai_{t} = softmax(hd_{t_{d}}^TH_{e}) \\
ci_{t} = \sum_{t_{e}}{ai_{t} hd_{t_{d}}} \\
hd^{'}_{t_{d}} = \tanh(Wi_{a} [hd_{t_{d}},ci_{t}])
\end{gathered}
\end{equation}
where $ai_{t}$ is a vector containing weights for all time steps of the encoder with respect to time step $t$ of the decoder, $H_{e}$ is the whole hidden states of the encoder, $ci_{t}$ is the weighted average of all hidden states of the encoder with respect to $hd_{t_{d}}$, $h^{'}_{d_{t}}$ is the desired hidden state of the decoder at time step $t$ that contains the correlated information from the encoder. 

Since trading volume is an important measure for the relative worth of market movement, time steps with high trading volume might carry more informative latent features. It is thus worth using self-attention mechanism \cite{cheng2016long} to highlight hot spots in both the encoder and decoder. Formally:
\begin{equation}
\begin{gathered}\label{eq:self-attention}
as_{t} = softmax(h_{t}^TH^{'}_{1:t-1}) \\
cs_{t} = \sum^{i=1}_{t-1}{as_{t_{i}} h_{t}} \\
h^{'}_{t} = \tanh(Ws_{a} [h_{t},cs_{t}])
\end{gathered}
\end{equation}
where $as_{t}$ is a vector containing weights for the hidden states of all previous time steps with respect to the hidden state at time step $t$, $cs_{t}$ is the weighted average of all hidden states of the previous time steps with respect to the hidden state at $t_{th}$ time step, $h^{'}_{t}$ is the desired hidden state at $t_{th}$ time step, and $H^{'}_{1:t-1}$ represents $[h^{'}_{1}, ..., h^{'}_{t-1}]$. The content-base measurement method is dot production, which is same as the inter-attention mechanism.

\subsection{Approximate posterior and stochasticity injection}
As mentioned in Section \ref{Introduction}, the adaptability is the main challenge to model financial markets trends. We use labelling methods to classify trends of financial markets to the following three classes: Up, Flat, and Down. However, labelling methods inevitably miss some useful information, such as specific values of Open, High, Low, Close price and Volume at each time step. For example, one of the common labelling methods is to first compute logarithm return between the close price at time step $t$ and $t+1$, and then compare the logarithm return with a given threshold to define the label at time step $t$. The sum of cross entropies between ground truth and predictions of target sequential data thus only represents how different the predicted disperse series of close price movement deviate from the true one. It turns out that, the variability of latent features is ignored by the training process of supervised sequential models in that the variability is an abstract representation of the original data rather than the labels. In other words, the penalties from cross entropies between softmax outputs and labels may have biases due to the fact that labels can not perfectly represent the intrinsic adaptability of financial trading data. 

To alleviate the above biases, we propose a unsupervised method to generate an extra regularizer. Inspired by the variational auto-encoder \cite{kingma2013auto,rezende2014stochastic}, which successfully learns efficient latent representations by fitting a recognition model to a approximate posterior, we introduce stochasticity into hidden states, the stochasticity can be trained by the reparameterization trick \cite{kingma2013auto} to form as the prior distribution of latent features. Meanwhile, following recent work about stochastic recurrent models \cite{bayer2014learning,chung2015recurrent,fraccaro2016sequential,goyal2017z}, we introduce a backward decoder to form the approximate posterior, then we apply the K-L divergence between the prior and posterior distribution as the extra regularizer to the objective function. 

%so that our model is able to take account to the adaptability of financial markets in that it can bring the models the extra penalties that incarnates the adaptability. We also follow recent work about stochastic recurrent models \cite{bayer2014learning,chung2015recurrent,fraccaro2016sequential,goyal2017z}, using a backward recurrent neural network to train the approximate posterior distribution.

According to the Bayesian paradigm and the variational lower bound, we assume financial trading historical data is a set of observed samples of a random variable $x$, the labels is a set of observed samples of a random variable $y$, the generation of $x$ and $y$ is conditioned by an unobserved random variable $z$ (we can regard $z$ as the abstract of the desired latent temporal features), which is generated by some random process parameterized by $\theta$. We train our model to attain the conditional probability distribution $p_{\theta}(y|x)$, which theoretically can be calculated by the integral of $p_{\theta}(y,z|x)$, formally,
\begin{equation}
\begin{gathered}\label{eq:post}
p_{\theta}(y|x) = \int{p_{\theta}(y,z|x)dz}
=\int{p_{\theta}(y|z,x)p_{\theta}(z|x)dz}
\end{gathered}
\end{equation}
however, it is intractable due to non-integrable $z$. A common approach is to use the variational lower bound $\mathcal{L}(x, \theta, \phi)$ to approximate $p_{\theta}(y|x)$,
\begin{equation}
\begin{gathered}\label{eq:ori_elbo}
\mathcal{L}(x, \theta, \phi)= \log p_{\theta}(y|x) - D_{KL}(p_{\phi}(z|x,y)||p_{\theta}(z|x,y))
\end{gathered}
\end{equation}
where $D_{KL}(p_{\phi}(z|x,y)||p_{\theta}(z|x,y))$ is the KLD between the approximate and true posterior. Following the approach by \cite{fraccaro2016sequential,goyal2017z}, we add a backward decoder to form the approximate posterior.

%Since KLD is non-negative, so the varaitional lower bound would approximate to desired log conditional $p_{\theta}(y|x)$ with KLD decreasing.  

Rewrite Equation (\ref{eq:ori_elbo}) in order for it to be differentiable,
\begin{equation}
\begin{gathered}\label{eq:alt_elbo}
\mathcal{L}(x, \theta, \phi)= \E_{p_{\phi}(z|x,y)}(\log p_{\theta}(y|x,z)) \\
- D_{KL}(p_{\phi}(z|x,y)||p_{\theta}(z|x))
\end{gathered}
\end{equation}
since we assume $\theta$ and $\phi$ are parameters of random process, we use two neural networks to form them, which can be trainable by the reparameterization trick. For the first term of Equation (\ref{eq:alt_elbo}), we sample the approximate posterior $p_{\phi}(z|x,y)$ to attain the latent variable $z$, then use it as one of the conditions for the log likelihood $\log p_{\theta}(y|x,z)$. Note that the approximate posterior is only used in the training procedure, the latent variable $z$ is from the $p_{\theta}(z|x)$ in the evaluation and test procedure. There would be no overfitting risks once DKL converges.

\subsection{The objective function}
%We introduce two sets of two-stack FC layers, denoting $FC_{\theta}$ and $FC_{\phi}$, to form the distribution $p_{\phi}(z|x,y)$ and $p_{\theta}(z|x)$. For the $p_{\theta}(z|x)$, we feed the hidden state $h_{t}$ of forward decoder separately into $FC_{\theta}$ to attain $z_{t}$. we use a group of FC and softmax layer to project hidden states of the forward decoder into probability distributions(the projection layers in left in Figure \ref{fig:CLVSA}). Following \cite{goyal2017z}, we also use another group of FC and softmax layer (the one in right) to attain an extra loss as the penalty for the backward decoder only for the sake of optimization.
The objective function of our model has the following three main parts: i) The cross entropies of predictions of the decoder, ii) The cross entropies of predictions of the backward decoder, iii) The KLD between the prior and posterior distribution, which are formed by the decoder and the backward decoder, respectively.

To extend Equation (\ref{eq:alt_elbo}) into the sequential scenario, we have the objective function as follows,
\begin{equation}
\begin{gathered}\label{eq:objective}
\mathcal{L}(x, \theta, \phi, \xi)= \sum_{t} \E_{p_{\phi}(z_{t}|x,y)}(\log p_{\theta}(y_{t}|x_{1:t},z_{1:t})) \\
+ \alpha \log p_{\xi}(y^{'}_{t}|b_{t}) \\
- \beta D_{KL}(p_{\phi}(z_{t}|x_{T:t},y^{'}_{t})||p_{\theta}(z_{t}|x_{1:t},z_{1:t-1})) + \gamma L_{2}
\end{gathered}
\end{equation}
where $\xi$ denotes the parameters of the projection layers for the backward decoder, $b_{t}$ denotes the hidden state of the backward decoder at the $t_{th}$ time stamp. $x_{T:t}$ and $y^{'}_{t}$ are the reversed trading data and the corresponding labels for the backward decoder, respectively. $\alpha$ and $\gamma$ denotes the weight of $p_{\xi}(y^{'}_{t}|b_{t}$ and $L_{2}$ regularizer, respectively. $\beta$ denotes the KLD annealing weight \cite{bowman2015generating}.

==> table.tex <==
\begin{table*}[!htp]
\centering
        \scalebox{0.72}{
            \begin{tabular}{*{19}{c|}}
                \cline{2-19}
                 & \multicolumn{3}{|c|}{CL}
                 & \multicolumn{3}{|c|}{NG}
                 & \multicolumn{3}{|c|}{GC}
                 & \multicolumn{3}{|c|}{S}
                 & \multicolumn{3}{|c|}{NQ}
                 & \multicolumn{3}{|c|}{ES}\\
                \cline{2-19}
                 & MAP & AAP & SP & MAP & AAP & SP & MAP & AAP & SP & MAP & AAP & SP & MAP & AAP & SP & MAP & AAP & SP \\
                \hline
                \multicolumn{1}{|c|}{$CNN_{s}$} & $43.8\%$ & $47.7\%$ & $1.55$ & $39.1\%$ & $37.0\%$ & $1.05$ & $35.6\%$ & $15.4\%$ & $0.67$ & $42.6\%$ & $44.3\%$ & $1.20$ & $45.1\%$ & $36.2\%$ & $1.54$ & $42.5\%$ & $33.8\%$ & $0.75$\\
                \multicolumn{1}{|c|}{$LSTM_{s}$} & $39.0\%$ & $41.4\%$ & $1.12$ & $40.0\%$ & $40.4\%$ & $1.23$ & $38.1\%$ & $21.1\%$ & $0.82$ & $40.1\%$ & $34.9\%$ & $1.13$ & $43.5\%$ & $32.2\%$ & $1.26$ & $40.0\%$ & $31.1\%$ & $0.62$\\
                
                \multicolumn{1}{|c|}{$Seq2Seq_{s}$} & $39.5\%$ & $39.4\%$ & $1.02$ & $39.6\%$ & $40.9\%$ & $1.11$ & $38.1\%$ & $20.8\%$ & $0.79$ & $40.2\%$ & $35.2\%$ & $1.17$ & $43.3\%$ & $32.7\%$ & $1.28$ & $40.3\%$ & $32.6\%$ & $0.67$ \\
                \hline
                \multicolumn{1}{|c|}{$CLSA$} & $47.8\%$ & $88.9\%$ & $2.69$ & $48.3\%$ & $60.1\%$ & $2.23$ & $43.7\%$ & $42.9\%$ & $1.08$ & $45.5\%$ & $54.2\%$ & $1.66$ & \pmb{$46.9\%$} & $41.8\%$ & $1.85$ & $44.3\%$ & $42.0\%$ & $1.02$ \\
                \hline
                \hline
                \multicolumn{1}{|c|}{$CLVSA$} & \pmb{$49.7\%$}  & \pmb{$113.0\%$} & \pmb{$3.99$} & \pmb{$50.7\%$} & \pmb{$73.7\%$} & \pmb{$3.01$} & \pmb{$45.5\%$} & \pmb{$50.2\%$} & \pmb{$1.58$} & \pmb{$48.0\%$} & \pmb{$57.6\%$} & \pmb{$1.81$} & $46.7\%$ & \pmb{$42.5\%$} & \pmb{$1.87$} & \pmb{$45.1\%$} & \pmb{$42.3\%$} & \pmb{$1.22$} \\
                \hline
                \end{tabular}
        }  
        \caption{Experimental results. MAP, AAP, and SP denote the mean average precision, average annual return, and Sharpe ratio, respectively. We ran each case five times to measure the robustness of each model. All values are average results of the repeated experiments.}
\label{tb:result}
\end{table*}
